In-beam performance of a Resistive Plate Chamber operated with eco-friendly gas mixtures

ALICE (A Large Ion Collider Experiment) studies the Quark-Gluon Plasma (QGP): a deconfined state of matter obtained in ultra-relativistic heavy-ion collisions. One of the probes for QGP study are quarkonia and open heavy flavour, of which ALICE exploits the muonic decay. A set of Resistive Plate Chambers (RPCs), placed in the forward rapidity region of the ALICE detector, is used for muon identification purposes. The correct operation of these detectors is ensured by the choice of the proper gas mixture. Currently they are operated with a mixture of C$_{2}$H$_{2}$F$_{4}$, i-C$_{4}$H$_{10}$ and SF$_{6}$ but, starting from 2017, new EU regulations have enforced a progressive phase-out of C$_{2}$H$_{2}$F$_{4}$ because of its large Global Warming Potential (GWP), making it difficult and costly to purchase. CERN asked LHC experiments to reduce greenhouse gases emissions, to which RPC operation contributes significantly. A possible candidate for C$_{2}$H$_{2}$F$_{4}$ replacement is the C$_{3}$H$_{2}$F$_{4}$ (diluted with other gases, such as CO$_{2}$), which has been extensively tested using cosmic rays. Promising gas mixtures have been devised; the next crucial steps are the detailed in-beam characterization of such mixtures as well as the study of their performance under increasing irradiation levels. This contribution will describe the methodology and results of beam tests carried out at the CERN GIF++ (equipped with a high activity $^{137}$Cs source and muon beam) with an ALICE-like RPC prototype, operated with several mixtures with varying proportions of CO$_{2}$, C$_{3}$H$_{2}$F$_{4}$, i-C$_{4}$H$_{10}$ and SF$_{6}$ . Absorbed currents, efficiencies, prompt charges, cluster sizes, time resolutions and rate capabilities will be presented, both from digitized (for detailed shape and charge analysis) and discriminated (using the same front-end electronics as employed in ALICE) signals.

==> authors.tex <==
%For corresponding author put a * after \author and its \affil and also the author's email after his name (e.g. if the corresponding author is Marcello you should put something like: 
%\author*[6,7] {\small M. Abbrescia}) \email{....@cern.ch}
%\affil*[\footnotesize 6]{\footnotesize Dipartimento Interateneo....
%\affil*[\footnotesize 7]{\footnotesize INFN Sezione di Bari....

%At least this is working for the EPJ plus template, for other journals it might be different
% \author{\small The RPC ECOgas@GIF++:} 

\author*[1]{\small \textbf{The RPC ECOgas@GIF++ Collaboration: }L. Quaglia} 
\author*[2,3]{\small D. Ramos} \email{\small dayron.ramos.lopez@cern.ch}
\author[6,3]{\small M. Abbrescia}
\author[21]{\small G. Aielli}
\author[3,8]{\small R. Aly}
\author[17]{\small M. C. Arena}
\author[11]{\small M. Barroso}
\author[4]{\small L. Benussi}
\author[4]{\small S. Bianco}
\author[7]{\small D. Boscherini}
\author[16]{\small F. Bordon}
\author[7]{\small A. Bruni}
\author[18]{\small S. Buontempo}
\author[16]{\small M. Busato}
\author[21]{\small P. Camarri}
\author[13]{\small R. Cardarelli}
\author[3]{\small L. Congedo}
\author[11]{\small D. De Jesus Damiao}
\author[6,3]{\small M. De Serio}
\author[21]{\small A. Di Ciacco}
\author[21]{\small L. Di Stante}
\author[14]{\small P. Dupieux}
\author[19]{\small J. Eysermans}
\author[12,1]{\small A. Ferretti}
\author[6,3]{\small G. Galati}
\author[12,1]{\small M. Gagliardi}
\author[12,1]{\small S. Garetti}
\author[16]{\small R. Guida}
\author[2,3]{\small G. Iaselli}
\author[14]{\small B. Joly}
\author[24]{\small S.A. Juks}
\author[23]{\small K.S. Lee}
\author[13]{\small B. Liberti} 
\author[22]{\small D. Lucero Ramirez}
\author[16]{\small B. Mandelli}
\author[14]{\small S.P. Manen}
\author[7]{\small L. Massa}
\author[3]{\small A. Pastore}
\author[13]{\small E. Pastori}
\author[4]{\small D. Piccolo}
\author[13]{\small L. Pizzimento}
\author[7]{\small A. Polini}
\author[13]{\small G. Proto}
\author[2,3]{\small G. Pugliese}
\author[16]{\small G. Rigoletti}
\author[13]{\small A. Rocchi}
\author[7]{\small M. Romano}
\author[10]{\small A. Samalan}
\author[9]{\small P. Salvini}
\author[21]{\small R. Santonico}
\author[5]{\small G. Saviano}
\author[13]{\small M. Sessa}
\author[6,3]{\small S. Simone}
\author[12,1]{\small L. Terlizzi}
\author[10,20]{\small M. Tytgat}
\author[12,1]{\small E. Vercellin}
\author[15]{\small M. Verzeroli}
\author[22]{\small N. Zaganidis}

\affil[\footnotesize 1]{\footnotesize INFN Sezione di Torino, Via P. Giuria 1, 10126 Torino, Italy}
\affil[\footnotesize 2]{\footnotesize Politecnico di Bari, Dipartimento Interateneo di Fisica, via Amendola 173, 70125 Bari, Italy}
\affil[\footnotesize 3]{\footnotesize INFN Sezione di Bari, Via E. Orabona 4, 70125 Bari, Italy}
\affil[\footnotesize 4]{\footnotesize INFN - Laboratori Nazionali di Frascati, Via Enrico Fermi 54, 00044 Frascati (Roma), Italy}
\affil[\footnotesize 5]{\footnotesize Sapienza Università di Roma, Dipartimento di Ingegneria Chimica Materiali Ambiente, Piazzale Aldo Moro 5, 00185 Roma, Italy}
\affil[\footnotesize 6]{\footnotesize Università degli studi di Bari, Dipartimento Interateneo di Fisica, via Amendola 173, 70125 Bari, Italy}
\affil[\footnotesize 7]{\footnotesize INFN Sezione di Bologna, Viale C. Berti Pichat 4/2, 40127 Bologna, Italy}
\affil[\footnotesize 8]{\footnotesize Helwan University, Helwan Sharkeya, Helwan, Cairo Governorate 4037120, Egypt}
\affil[\footnotesize 9]{\footnotesize INFN Sezione di Pavia, Via A. Bassi 6, 27100 Pavia, Italy}
\affil[\footnotesize 10]{\footnotesize Ghent University, Dept. of Physics and Astronomy, Proeftuinstraat 86, B-9000 Ghent, Belgium}
\affil[\footnotesize 11]{\footnotesize Universidade do Estado do Rio de Janeiro, R. São Francisco Xavier, 524 - Maracanã, Rio de Janeiro - RJ, 20550-013, Brasil}
\affil[\footnotesize 12]{\footnotesize Università degli studi di Torino, Dipartimento di Fisica, Via P. Giuria 1, 10126 Torino, Italy}
\affil[\footnotesize 13]{\footnotesize INFN Sezione di Roma Tor Vergata, Via della Ricerca Scientifica 1, 00133 Roma, Italy}
\affil[\footnotesize 14]{\footnotesize Clermont Université, Université Blaise Pascal, CNRS/IN2P3, Laboratoire de Physique Corpusculaire, BP 10448, F-63000 Clermont-Ferrand, France}
\affil[\footnotesize 15]{\footnotesize Université Claude Bernard Lyon I, 43 Bd du 11 Novembre 1918, 69100 Villeurbanne, France}
\affil[\footnotesize 16]{\footnotesize CERN, Espl. des Particules 1, 1211 Meyrin, Svizzera}
\affil[\footnotesize 17]{\footnotesize Università degli studi di Pavia, Corso Strada Nuova 65, 27100 Pavia, Italy}
\affil[\footnotesize 18]{\footnotesize INFN Sezione di Napoli, Complesso Universitario di Mone S. Angelo ed. 6, Via Cintia, 80126 Napoli, Italy}
\affil[\footnotesize 19]{\footnotesize Massachusetts Institute of Technology, 77 Massachusetts Ave, Cambridge, MA 02139, USA}
\affil[\footnotesize 20]{\footnotesize Vrije Universiteit Brussel (VUB-ELEM), Dept. of Physics, Pleinlaan 2, 1050 Brussels, Belgium}
\affil[\footnotesize 21]{\footnotesize Università degli studi di Roma Tor Vergata, Dipartimento di Fisica, via della Ricerca Scientifica 1, 00133 Roma, Italy }
\affil[\footnotesize 22]{\footnotesize Universidad Iberoamericana, Dept. de Fisica y Matematicas, Mexico City 01210, Mexico.}
\affil[\footnotesize 23]{\footnotesize Korea University, 145 Anam-ro, Seongbuk-gu, Seoul, South Korea}
\affil[\footnotesize 24]{\footnotesize Université Paris-Saclay, 3 rue Joliot Curie, Bâtiment Breguet 91190 Gif-sur-Yvette, France}
